Ego-Network Transformer for Subsequence Classification in Time Series Data

Time series classification is a widely studied problem in the field of time series data mining. Previous research has predominantly focused on scenarios where relevant or foreground subsequences have already been extracted, with each subsequence corresponding to a single label. However, real-world time series data often contain foreground subsequences that are intertwined with background subsequences. Successfully classifying these relevant subsequences requires not only distinguishing between different classes but also accurately identifying the foreground subsequences amidst the background. To address this challenge, we propose a novel subsequence classification method that represents each subsequence as an ego-network, providing crucial nearest neighbor information to the model. The ego-networks of all subsequences collectively form a time series subsequence graph, and we introduce an algorithm to efficiently construct this graph. Furthermore, we have demonstrated the significance of enforcing temporal consistency in the prediction of adjacent subsequences for the subsequence classification problem. To evaluate the effectiveness of our approach, we conducted experiments using 128 univariate and 30 multivariate time series datasets. The experimental results demonstrate the superior performance of our method compared to alternative approaches. Specifically, our method outperforms the baseline on 104 out of 158 datasets.

==> insert/fig_3nn_graph.tex <==
\begin{figure}[ht]
\centerline{
\includegraphics[width=0.99\linewidth]{insert/figure/fig_3nn_graph_1.pdf}
}
\caption{
An example of a 3-nearest neighbor subsequence graph is shown, with the target subsequence represented by the green \textit{input} node.
}
\label{fig:3nn_graph}
\end{figure}


==> insert/fig_block.tex <==
\begin{figure}[ht]
\centerline{
\includegraphics[width=0.99\linewidth]{insert/figure/fig_block_0.pdf}
}
\caption{
The designs of the residual block, \protect\mybox{\texttt{RBlock}}, and the Transformer block, \protect\mybox{\texttt{TBlock}}, are shown in this figure.
}
\label{fig:block}
\end{figure}


==> insert/tab_egonet.tex <==
\begin{table}[ht]
\caption{Utilizing ego-networks improves performance.}
\begin{center}
\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{l||c|cc|c|cc}
\multirow{3}{*}{Avg. rank ($\downarrow$)} & \multicolumn{3}{c|}{\textbf{UCR}} & \multicolumn{3}{c}{\textbf{UEA}} \\ \cline{2-7}
~ & \multirow{2}{*}{\textbf{Baseline}} & \multicolumn{2}{c|}{\textbf{Ego-net}} & \multirow{2}{*}{\textbf{Baseline}} & \multicolumn{2}{c}{\textbf{Ego-net}} \\ 
~ &  & 5NN & 10NN & ~ & 5NN & 10NN \\ \hline \hline
LSTN & 10.65 & 7.35 & 7.61 & 8.58 & 7.58 & 7.15  \\ 
GRU & 9.18 & 7.15 & 7.34 & 8.62 & 8.23 & 7.50  \\ 
ResNet & 4.30 & 3.68 & 3.73 & 5.58 & 5.12 & 4.80  \\ 
Transformer & 7.09 & 4.87 & 5.06 & 5.90 & 4.87 & 4.07  \\ \hline
Average & 7.81 & 5.76 & 5.93 & 7.17 & 6.45 & 5.88 \\ 
\end{tabular}
}
\label{tab:egonet}
\end{center}
\end{table}


==> insert/tab_smooth.tex <==
\begin{table}[ht]
\caption{The post-processing step improves performance.}
\begin{center}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{l||cc|cc}
\multirow{2}{*}{Avg. rank ($\downarrow$)} & \multicolumn{2}{c|}{\textbf{UCR}} & \multicolumn{2}{c}{\textbf{UEA}} \\ \cline{2-5}
~ & \textbf{Before} & \textbf{After} & \textbf{Before} & \textbf{After}  \\ \hline \hline
1NN & 13.36 & 7.03 & 12.60 & 9.63  \\ 
5NN & 11.76 & 7.56 & 11.65 & 9.50  \\ 
10NN & 12.35 & 8.87 & 11.43 & 9.53  \\ 
$k$NN & 11.90 & 7.03 & 11.13 & 9.12  \\ \hline
LSTN & 11.97 & 10.28 & 9.10 & 6.97  \\ 
GRU & 9.32 & 7.38 & 8.98 & 7.17  \\ 
ResNet & 3.34 & 2.68 & 4.95 & 3.67  \\
Transformer & 6.52 & 4.64 & 6.43 & 4.13 \\ \hline
Average & 10.07 & 6.93 & 9.54 & 7.46 \\
\end{tabular}
}
\label{tab:smooth}
\end{center}
\end{table}


==> section/method.tex <==
\section{Models and Methodology}
\label{sec:model}
In this section, we begin by introducing the proposed method for classifying an input subsequence ego-network.
Next, we present the backbone models utilized to extract representations from the input time series data.
Then, we describe the training and inference algorithm associated with the proposed model.
Lastly, we discuss a simple yet effective post-processing technique designed to enhance the temporal consistency in the prediction of adjacent subsequences.

\subsection{Ego-network Transformer Model}
\label{sec:ego_model}
The proposed Transformer model is presented in Fig.~\ref{fig:egonet}. 
The input to the model consists of a focal subsequence denoted as $X_\text{focal}$, along with its nearest neighbor subsequences from the training time series $X_0, \cdots, X_{k-1}$, and the corresponding labels of the neighbors $y_{0}, \cdots, y_{k-1}$.
Essentially, the inputs consist of the subsequences associated with the ego-network of the focal subsequence, where the ego-network is extracted from the $k$-nearest neighbor subsequence graph.
The initial step involves extracting the intermediate representation of each subsequence using one of the backbone models discussed in Section~\ref{sec:backbone}. 
These representations are denoted as $H_\text{focal}, H_0, H_1, \cdots, H_{k-1}$, where $H_\text{focal}$ corresponds to the representation of $X_\text{focal}$, and $H_0, H_1, \cdots, H_{k-1}$ correspond to the representations of $X_0, X_1, \cdots, X_{k-1}$, respectively.

\input{insert/fig_egonet}

Next, we incorporate the corresponding label for each neighbor subsequence by adding a learnable label embedding to its representation. 
Let $Y_i$ represent the label embedding for $y_i$, the label of the $i$th neighbor. 
The final subsequence representation for the neighbor is computed as $\hat{H}_i \gets Y_i + H_i$.
With the node representations of each subsequence prepared, we concatenate them together to form a set that includes all the node representations: $[H_\text{focal}, \hat{H}_0, \cdots, \hat{H}_{k-1}]$.
Subsequently, we employ two layers of Transformer blocks (refer to Fig.~\ref{fig:tblock}) to aggregate information from each node in the set.
After the Transformer blocks, we extract the representation corresponding to the focal subsequence. 
Finally, a linear layer is used to compute the logit for each class.
We choose to use a Transformer-based model design to capture the ego-network, as opposed to other graph neural networks like GCN~\cite{kipf2016semi} or GAT~\cite{velivckovic2017graph}, because it has been shown in~\cite{ying2021transformers} that Transformers are more effective compared to the alternatives.

The proposed method leverages the versatile and powerful $k$-nearest neighbor subsequence graph, as discussed in Section~\ref{sec:ts_graph}, for the subsequence classification problem. 
This approach offers notable advantages over attending to all subsequences in the training data. 
By focusing only on the top $k$ nearest neighbors, the method achieves improved efficiency. 
This is particularly significant considering the space complexity of the Transformer block, which grows quadratically with the number of input items. 
For instance, if the training data consists of one million subsequences, storing the attention matrix alone would require over seven terabytes of memory.

\subsection{Backbone Temporal Model}
\label{sec:backbone}
We have explored four different neural network architectures as backbone models for extracting global representations from time series data. 
A global representation captures the information from the entire input time series. 
The four backbone models are:

\begin{itemize}
\item The \textbf{Long Short-Term Memory Network (LSTM)} is a widely used type of Recurrent Neural Network (RNN) for modeling sequential data~\cite{hochreiter1997long,lim2021time,zhou2021informer}.
In our work, we adopt the design depicted in Fig.~\ref{fig:backbone}.a.
The figure employs specific notations to describe different layers. 
For instance, \mybox{\texttt{1D conv,7/2,$n_\text{in}{\to}$64}} represents a $1D$ convolutional layer with a filter size of 7, a stride size of 2, an input dimension of $n_\text{in}$, and an output dimension of 64.
Similarly, \mybox{\texttt{bi-RNN,64${\to}$64}} denotes a bidirectional RNN layer with an input dimension of 64 and an output dimension of 64.
In our case, the two bi-RNN layers are implemented as bidirectional LSTM layers.
Additionally, \mybox{\texttt{linear,64${\to}$64}} denotes a linear layer with an input dimension of 64 and an output dimension of 64.

\forceindent Initially, the input time series is processed by the $1D$ convolutional layer to extract local patterns.
Subsequently, the two bidirectional LSTM layers summarize the input sequence using the LSTM recurrent mechanism.
The output of the last LSTM layer is a sequence of vectors, each with a size of 64. 
From this output sequence, we extract the vector corresponding to the last time step. 
This selected vector is then passed through three linear layers, with ReLU activation layers in between.
The decision to select only the last time step is based on the understanding that it encapsulates the information from the entire input time series. 
However, it is worth noting that the first time step could also be chosen since the RNN layers are bidirectional. 
In the end, the output of the LSTM backbone model consists of a size 128 vector for each input time series.

\item The \textbf{Gated Recurrent Unit Network (GRU)} is another popular type of RNN architecture for modeling sequential data~\cite{cho2014properties,lim2021time,zhou2021informer}.
We employ an identical design to the LSTM backbone model (see Fig.~\ref{fig:backbone}.a), with the only difference being that the two bi-RNN layers are implemented as GRU layers instead of LSTM layers.

\item The \textbf{Residual Network (ResNet)} is a time series classification model inspired by the success of ResNet in computer vision~\cite{he2016deep, wang2017time}. 
Extensive evaluations reported in~\cite{ismail2019deep} have demonstrated that ResNet is one of the most effective models for time series classification. 
Our design, depicted in Fig.\ref{fig:backbone}.b, is based on the architecture proposed in~\cite{wang2017time}. 
In our notation, \mybox{\texttt{RBlock,64$\to$64}} represents a residual block (refer to Fig.\ref{fig:rblock}) with an input dimension of 64 and an output dimension of 64.

\forceindent Similar to the RNN-based model, the initial layer in the ResNet architecture is a $1D$ convolutional layer responsible for capturing low-level local patterns. 
Subsequently, the output of the $1D$ convolutional layer is passed through three residual blocks. 
The design of the residual block is illustrated in Fig.~\ref{fig:rblock} and will be further explained in a subsequent paragraph. 
The length of the output sequence from the residual blocks depends on the length of the input time series. 
When the sequence length is greater than one, we employ a global average pooling function to generate a global intermediate representation of the input time series. 
This global intermediate representation is then processed by three linear layers with ReLU activation functions. 
Ultimately, the output of this backbone model is a size 128 vector that represents each input time series.

\item The \textbf{Transformer} is a widely adopted alternative to RNNs for sequence modeling~\cite{vaswani2017attention, li2019enhancing, zhou2021informer, lim2021time, chen2022denoising}.
In our work, we adopt the architecture depicted in Fig.\ref{fig:backbone}.c. 
Like the previously discussed backbone models, the initial layer comprises a $1D$ convolutional layer designed to capture local patterns. 
To incorporate positional information, we follow~\cite{vaswani2017attention} and apply fixed positional encoding.
This encoding is added to the output of the $1D$ convolutional layer. 
Furthermore, to enable effective learning of global representations for the input time series, we prepend a special token \texttt{[start]} to the beginning of the sequence.

\forceindent Next, the input sequence passes through four consecutive Transformer blocks, denoted as \mybox{\texttt{TBlock,8,64${\to}$64}}.
In this notation, the number 8 refers to the attention heads, and the two 64 values represent the input and output dimensions, respectively. 
The design of the Transformer block is visually represented in Fig.~\ref{fig:tblock}, and in the subsequent paragraph, we will provide a detailed explanation of its design. 
From the output sequence generated by the Transformer blocks, we extract the intermediate representation associated with the \texttt{[start]} token. 
This extracted representation serves as the global representation of the input time series, capturing the essential information from the entire sequence.
This mechanism shares similarities with the \texttt{[CLS]} token used in prior Transformer models like BERT~\cite{devlin2018bert}, highlighting its significance in capturing global context. 
Subsequently, the global intermediate representation undergoes processing through three linear layers, with the first two followed by a ReLU activation function. 
Finally, the output of this backbone model is a size 128 vector that represents each input time series.

\end{itemize}

\input{insert/fig_backbone}

The detailed design of the residual block can be found in Fig.~\ref{fig:rblock}. 
This block consists of two passages: the main passage and the skip connection passage. 
The main passage processes the input sequence using three pairs of $1D$ convolutional-ReLU layers. 
The convolutional layers have filter sizes of seven, five, and three, sequentially, progressing from the input to the output.
On the other hand, the skip connection passage may include an optional $1D$ convolutional layer with a filter size of one. 
This convolutional layer is only introduced to the skip connection when the input dimension and the output dimension of the residual block differ.
The output of the main passage and the skip connection passage are combined through element-wise addition to form the final output of the block. 

\input{insert/fig_rblock}

The design of the Transformer block is illustrated in Fig.\ref{fig:tblock}, showcasing its structure and components. 
The Transformer block is composed of two stages: a multihead self-attention stage and a feed-forward stage.
In the first stage, a multihead self-attention module is employed. 
This module allows the Transformer block to capture dependencies between different positions in the input sequence.
The second stage involves a position-wise feed-forward network. 
This network applies two linear layers with a ReLU activation function to each position of the sequence obtained from the multihead self-attention module.
This stage enables the Transformer block to incorporate non-linear transformations and enhance the representation of each position.
Both stages incorporate skip connections, ensuring that the input is added to the output at each stage. 
This mechanism facilitates the flow of information from the input to the output, enabling the model to retain important information throughout the block.
The Transformer block is responsible for modeling complex dependencies and enhancing the representation of the input sequence through self-attention and position-wise transformations.

\input{insert/fig_tblock}

We adopt layer normalization~\cite{ba2016layer} for all normalization layers in our model. 
Layer normalization has proven to be effective and is commonly used with sequential data~\cite{ba2016layer,vaswani2017attention}. 
By applying layer normalization, we can ensure stable and consistent normalization across different layers.

\subsection{Model Training and Inference}
The training procedure for the proposed ego-network Transformer model is outlined in Algorithm~\ref{alg:train}. 
The algorithm takes the following inputs: the training time series $T$, the ground truth labels $Y$, the subsequence length $m$, and the number of neighbors $k$.

\input{insert/alg_train}

To begin, in line 2, Algorithm~\ref{alg:knn_stomp} is employed to construct the $k$-nearest neighbor graph $\mathcal{G}$.
Next, in line 4, the number of samples $n_\text{sample}$ is calculated. 
This value corresponds to the minimal number of subsequences used for training in each epoch and is determined based on the number of subsequences required to cover the time series $T$.
Using all subsequences would lead to redundancy due to overlap between subsequences.
In line 5, $n_\text{sample}$ subsequences are randomly sampled from $T$ without replacement.
The sampling process yields the sampled subsequences $\mathbf{X}_\text{sample}$, their associated ground truth labels $Y_\text{sample}$, and the indices of the subsequences $I_\text{sample}$.
This random sampling approach enables the model to train on different shifts of essentially the same subsequences, thereby enhancing its robustness.

In line 7, the mini-batch for the iteration is prepared, consisting of the subsequence $\mathbf{X}_\text{batch}$, the corresponding ground truth labels $Y_\text{batch}$, and the indices $I_\text{batch}$.
In line 8, by utilizing the $k$-nearest neighbor graph $\mathcal{G}$ and the indices $I_\text{batch}$, we obtain the indices of the $k$-neighbors, denoted as $\mathbf{I}_\text{neighbor}$, for each sample in the mini-batch.
It is important to note that $\mathbf{I}_\text{neighbor}$ is a matrix of size $n_\text{batch} \times k$, where $\mathbf{I}_\text{neighbor}[i, j]$ contains the index of the $j$th neighbor for the $i$th sample in the mini-batch.
In line 9, we extract the subsequences and labels for each neighbor based on the indices in $\mathbf{I}_\text{neighbor}$.
Line 10 involves updating the parameters $\theta$ of the ego-network Transformer model $f_\theta$.
Finally, in line 11, the trained model $f_\theta$ is returned as the output of the algorithm.

The inference procedure for the proposed Transformer model is presented in Algorithm~\ref{alg:inference}.
The algorithm accepts the following inputs: the test time series $T_\text{test}$, the training time series $T_\text{train}$, the training labels $Y_\text{train}$, the subsequence length $m$, and the number of neighbors $k$.

\input{insert/alg_inference}

Similar to Algorithm~\ref{alg:train}, Algorithm~\ref{alg:inference} also constructs the $k$-nearest neighbor graph $\mathcal{G}$ in line 2, but with the difference that it finds the $k$-nearest neighbors from $T_\text{train}$ for each subsequence in $T_\text{test}$.
From line 3 to line 6, the algorithm predicts the label for each subsequence $\mathbf{X}_i \in T_\text{test}$, where $i$ denotes the index associated with $\mathbf{X}_i$.
In line 4, the index of the neighbors for the subsequence $\mathbf{X}_i$ is extracted from $\mathcal{G}$.
In line 5, the subsequence and label for each neighbor are extracted from $T_\text{train}$ and $Y_\text{train}$.
In line 6, the label for $\mathbf{X}_i$ is predicted and stored in $\hat{Y}_\text{test}[i]$.
The predicted labels $\hat{Y}_\text{test}$ are returned in line 7.

It's worth noting that although we introduced both Algorithm~\ref{alg:train} and Algorithm~\ref{alg:inference} with univariate time series, both algorithms can also handle multivariate time series.

\subsection{Temporal Consistency Post-processing}
To ensure temporal consistency, we employ a sliding window technique to smooth the predicted label series. 
This post-processing method is both simple and effective. 
By following these steps, we obtain the smoothed label vector $Y_\text{after}$ from the input label vector $Y_\text{before}$ and a sliding window length $m$:

\begin{enumerate}
    \item Starting from the left and progressing towards the right, we identify the next onset for the relevant classes (i.e., non-background classes) in $Y_\text{before}$.
    \item If an onset is found at index $i_\text{onset}$, we determine the majority class within $Y_\text{before}[i_\text{onset}:i_\text{onset} + m]$.
    \item If the majority class identified in the previous step is denoted as $c$, we assign $c$ to $Y_\text{after}[i_\text{onset}:i_\text{onset} + m]$.
    \item Repeat steps 1--3 until reaching the end.
\end{enumerate}

Figure~\ref{fig:smooth} provides a visual example illustrating the post-processing method with $m=3$. 
In this example, three onsets (\texttt{onset 0}, \texttt{onset 1}, and \texttt{onset 2}) are detected, and there are three classes (\texttt{class 0} which represents the background, \texttt{class 1}, and \texttt{class 2}). 
For \texttt{onset 0}, the majority class within the window is \texttt{class 1}, so we set the corresponding values in $Y_\text{after}$ to \texttt{class 1}. 
Similarly, for \texttt{onset 1} and \texttt{onset 2}, we assign the corresponding values in $Y_\text{after}$ as \texttt{class 2} and \texttt{class 0}, respectively. 
This post-processing method improves the temporal consistency of the predicted labels. 
In the given example, the likely erroneous classification of \texttt{class 1} at \texttt{onset 2} is corrected. 
Please note that in our experiments, we determine the length of the sliding window using a validation dataset.

\input{insert/fig_smooth}

